A Noncrossing Basis for Noncommutative Invariants of SL(2,C)

Noncommutative invariant theory is a generalization of the classical invariant theory of the action of $SL(2,\IC)$ on binary forms. The dimensions of the spaces of invariant noncommutative polynomials coincide with the numbers of certain noncrossing partitions. We give an elementary combinatorial explanation of this fact by constructing a noncrossing basis of the homogeneous components. Using the theory free stochastic measures this provides a combinatorial proof of the Molien-Weyl formula in this setting.

==> Invariants-10_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=2.499539 -12.804428 87.538909 9.946448]{Invariants-10_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-80.915173,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-73.963166,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-67.011159,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-60.059152,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-53.107144,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-46.155137,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-39.203130,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-32.251123,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-25.299116,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-18.347109,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-11.395102,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){3}


==> Invariants-11_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=2.499539 -12.804428 87.538909 9.946448]{Invariants-11_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-80.915173,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-73.963166,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-67.011159,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-60.059152,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-53.107144,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-46.155137,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-39.203130,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-32.251123,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-25.299116,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-18.347109,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-11.395102,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){3}


==> Invariants-12_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=10.810780 -12.804428 95.850150 12.439821]{Invariants-12_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-80.915173,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-65.620757,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-50.326342,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-35.031926,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-19.737511,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){3}


==> Invariants-1_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=10.810780 -12.804428 95.850150 12.439821]{Invariants-1_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-80.915173,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-65.620757,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-50.326342,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-35.031926,9.238945)(-0.500000,-1.000000){4}
\ASYalign(-19.737511,9.238945)(-0.500000,-1.000000){5}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){6}


==> Invariants-2_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=10.810780 -12.804428 95.850150 12.439821]{Invariants-2_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-80.915173,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-65.620757,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-50.326342,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-35.031926,9.238945)(-0.500000,-1.000000){4}
\ASYalign(-19.737511,9.238945)(-0.500000,-1.000000){5}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){6}


==> Invariants-3_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 11.455249]{Invariants-3_0.eps}%


==> Invariants-4_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 7.253281]{Invariants-4_0.eps}%


==> Invariants-5_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 11.455249]{Invariants-5_0.eps}%


==> Invariants-6_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 11.455249]{Invariants-6_0.eps}%


==> Invariants-7_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 11.455249]{Invariants-7_0.eps}%


==> Invariants-8_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=13.756562 -0.250000 56.276247 7.253281]{Invariants-8_0.eps}%


==> Invariants-9_.tex <==
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\setlength{\unitlength}{1pt}
\includegraphics[bb=5.076489 -12.804428 118.462316 13.554179]{Invariants-9_0.eps}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-109.367929,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-99.829307,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-90.290686,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-80.752065,9.238945)(-0.500000,-1.000000){1}
\ASYalign(-71.213444,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-61.674822,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-52.136201,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-42.597580,9.238945)(-0.500000,-1.000000){2}
\ASYalign(-33.058959,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-23.520337,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-13.981716,9.238945)(-0.500000,-1.000000){3}
\ASYalign(-4.443095,9.238945)(-0.500000,-1.000000){3}

